Does BLEU Score Work for Code Migration?

Statistical machine translation (SMT) is a fast-growing sub-field of computational linguistics. Until now, the most popular automatic metric to measure the quality of SMT is BiLingual Evaluation Understudy (BLEU) score. Lately, SMT along with the BLEU metric has been applied to a Software Engineering task named code migration. (In)Validating the use of BLEU score could advance the research and development of SMT-based code migration tools. Unfortunately, there is no study to approve or disapprove the use of BLEU score for source code. In this paper, we conducted an empirical study on BLEU score to (in)validate its suitability for the code migration task due to its inability to reflect the semantics of source code. In our work, we use human judgment as the ground truth to measure the semantic correctness of the migrated code. Our empirical study demonstrates that BLEU does not reflect translation quality due to its weak correlation with the semantic correctness of translated code. We provided counter-examples to show that BLEU is ineffective in comparing the translation quality between SMT-based models. Due to BLEU's ineffectiveness for code migration task, we propose an alternative metric RUBY, which considers lexical, syntactical, and semantic representations of source code. We verified that RUBY achieves a higher correlation coefficient with the semantic correctness of migrated code, 0.775 in comparison with 0.583 of BLEU score. We also confirmed the effectiveness of RUBY in reflecting the changes in translation quality of SMT-based translation models. With its advantages, RUBY can be used to evaluate SMT-based code migration models.

==> body.tex <==
\section{Proposal}
\section{Related Works}






==> gved.tex <==
\subsubsection{\textbf{Graph Vector Edit Distance (GVED)}}

Graph-based approaches in representing program semantics have become
popular. Among those approaches, PDGs are one of the most popular.  To
capture the graph structures in PDGs, we choose Exas~\cite{fase09}.
Exas is an efficient structural characteristic feature extraction
approach that approximates and captures the structure within the
fragments of artifacts~\cite{fase09}.  In our study, we use Exas as a
mean of computing the difference between two PDGs. Given a pair of
method in C\# which are need to be compared, their respective
(PDGs) are built.
% with some additional nodes from GROUM~\cite{fse09}.
Exas vectors will be computed on those graphs. In Exas, the
characteristic features are extracted from the patterns of elements of
the graphs. The code fragments are characterized by their counting
vectors of those features. The difference between two vectors reflects
the difference of two graphs.

%Therefore, distance of these counting vectors is considered the way to measure the sematic between code fragments.

Figure~\ref{fig:PDGs} shows the PDGs of the code fragments 1 and
2. These graphs are analysed by Exas, which focuses on two kinds of
patterns of structural information of the graph, called $\left(p,q\right)$-node
and $n$-path as can be seen in Table~\ref{tab:feature1} and
Table~\ref{tab:feature2}.

An efficient way to express the property ``having the same or similar
features'' is to use vectors. The characteristic vector of a fragment
is the occurrence-count vector of its features. That is, each position
in the vector is indexed for a feature and the value at that position
is the number of occurrences of that feature in the
fragment. Table~\ref{tab:featureIndex} shows the indexes of the
features, which are global across all vectors. Based on the occurrence
counts, the vectors for code fragment 1 and~2 are
$V_1$(1,1,1,1,1,0,1,0...) and $V_2$(1,1,0,1,1,1,1,1...),
respectively. Two fragments having the same feature sets and
occurrence counts will have the same vectors. The
vector similarity can be measured by a chosen vector distance such as
1-norm distance.

We introduce the formula for normalizing the result of vector edit
distance which is used in our experiments. The normalized
value is described as
\[GVED \left( V_1, V_2 \right) = 1 - \sum_{i=1}^{n} \frac{ \mid XV1_i - XV2_i \mid}{XV1_i + XV2_i}\]
where $n$ denotes the number of vector scalar, $V_1$ denotes the
counting vector of the first graph, $V_2$ denotes the counting vector
of the second graph; $XV1_i$ denotes the value of the ($i-th$) scalar
of $V_1$; and $XV2_i$ denotes the value of the ($i-th$) scalar of
$V_2$.

In this example in Figure~\ref{code1code2}, the value of GVED is
$GVED\left(V_1, V_2\right) = 1 - \frac{8 }{20} = 0.6 $.

\begin{figure}
\begin{lstlisting}[language=JAVA]
	Code 1:
	void foo(int i) {
		int j;
		if (i < 2) {
			j = 1;
		} else {
			j = 2;
		}
	}

	Code 2:
	void foo(int i) {
		int j;
		if (i < 2)
			j = i;	
		j = 2;
	}
\end{lstlisting}
\caption{Example of two code fragments}
\label{code1code2}
\end{figure}

\begin{figure}[t]
	\caption{An example: two PDGs represent code fragments 1 and 2}
	\includegraphics[scale=0.4]{img/Diagram_PDG.png}
	\centering
	\label{fig:PDGs}
\end{figure}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{Feature Table of Code Fragment 1 in Exas}
  \scalebox{0.65}{
    \begin{tabular}{|l|l|l|l|l|r|}
    \toprule
    \textbf{Pattern} & \multicolumn{5}{c|}{\textbf{Feature of Code1}} \\
    \midrule
    \textit{\textbf{1-path}} & inputInt & intSmall2 & intEqual1 & intEqual2 & \multicolumn{1}{l|}{declareInt} \\
    \midrule
    \textit{\textbf{2-path}} & \multicolumn{1}{p{6.415em}|}{inputInt-intSmall2} & \multicolumn{1}{p{5.915em}|}{intSmall2-intEqual1} & \multicolumn{1}{p{6em}|}{intSmall2-intEqual2} & \multicolumn{1}{p{5.75em}|}{declareInt-intEqual1} & \multicolumn{1}{p{5em}|}{declareInt-intEqual2} \\
    \midrule
    \textit{\textbf{3-path}} & \multicolumn{1}{p{6.415em}|}{intputInt-intSmall2-intEqual1} & \multicolumn{1}{p{5.915em}|}{intputInt-intSmall2-intEqual2} &       &       &  \\
    \midrule
    \textit{\textbf{(p,q)-node}} & inputInt-0-1 & intSmall2-1-2 & intEqual1-2-0 & intEqual2-1-2 &  \\
    \bottomrule
    \end{tabular}%
	}
  \label{tab:feature1}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
	\caption{Feature Table of Code Fragment 2 in Exas}
	\scalebox{0.65}{
	    \begin{tabular}{|l|l|l|l|l|r|}
    \toprule
    \textbf{Pattern} & \multicolumn{5}{c|}{\textbf{Feature of Code2}} \\
    \midrule
    \textit{\textbf{1-path}} & inputInt & intSmall2 & intEqualInt & intEqual2 & \multicolumn{1}{l|}{declareInt} \\
    \midrule
    \textit{\textbf{2-path}} & \multicolumn{1}{p{6.415em}|}{inputInt-intSmall2} & \multicolumn{1}{p{5.915em}|}{intSmall2-intEqualInt} & \multicolumn{1}{p{6em}|}{declareInt-intEqual1} & \multicolumn{1}{p{5.75em}|}{declareInt-intEqual2} &  \\
    \midrule
    \textit{\textbf{3-path}} & \multicolumn{1}{p{6.415em}|}{intputInt-intSmall2-intEqualInt} &       &       &       &  \\
    \midrule
    \textit{\textbf{(p,q)-node}} & inputInt-0-1 & intSmall2-1-1 & intEqualInt-2-0 & intEqual2-1-0 &  \\
    \bottomrule
    \end{tabular}%
	}
  \label{tab:feature2}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
	\centering
	\caption{Feature Indexing}
	\scalebox{0.75}{
	\begin{tabular}{|cccc|}
		\toprule
		\multicolumn{1}{|l|}{\textbf{Feature}} & \multicolumn{1}{l|}{\textbf{Index}} & \multicolumn{1}{l|}{\textbf{Counted in Code1}} & \multicolumn{1}{l|}{\textbf{Counted in Code2}} \\
		\midrule
		\multicolumn{1}{|l|}{inputInt} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{intSmall2} & \multicolumn{1}{r|}{2} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{intEqual1} & \multicolumn{1}{r|}{3} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{0} \\
		\midrule
		\multicolumn{1}{|l|}{intEqual2} & \multicolumn{1}{r|}{4} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{declareInt} & \multicolumn{1}{r|}{5} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{intEqualInt} & \multicolumn{1}{r|}{6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|p{5.75em}|}{inputInt-intSmall2} & \multicolumn{1}{r|}{7} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{intEqual2-1-0} & \multicolumn{1}{r|}{8} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{4}{|c|}{To be continued} \\
		\bottomrule
	\end{tabular}%
	}
	\label{tab:featureIndex}%
\end{table}%


==> treed.tex <==
\subsection{Code similarity metrics}

\subsubsection{\textbf{String Edit Distance (SED)}}
String Edit Distance (SED) is the metric to compare source code when
it is represented as sequence of tokens. SED measures efforts that a
user must edit in term of the tokens that need to be deleted/added to
transform the resulting code into the correct one. In our study, we
used Levenshtein algorithm to calculate that distance. The metric is
normalized as: $SED = 1 - \frac{EditDistance\left(s_R,
  s_T\right)}{length\left(s_R\right)}$ where $s_R$ is the sequence of
tokens representing the reference code; $s_T$ is the sequence of
tokens represent the translated code; $EditDistance\left(s_R,
s_T\right)$ is the editing distance between the pair; and the
denominator is the total length of the reference code. For example,
$EditDistance\left(s_R, s_T\right)$ between translated code and
reference code in Figure~\ref{fig:issueexample2} is 4 (two deletions,
two additions). Then, it is normalized as 0.952. Note that the closer
the score to 1, the more similar the pair in term of lexical~tokens.

\subsubsection{\textbf{Tree Edit Distance (TREED)}}  

Abstract syntax tree (AST) is the most widely-used representation in
representing the syntactic structures in source code. Therefore,
computing the difference of two ASTs is considered as evaluating
syntactic difference.  In our study, we apply this idea in measuring
the difference between the syntactic structures of reference code and
translated code. Given a pair of methods in C\# which are need to be
syntactically compared, we used Roslyn~\cite{roslyn} to parse them into
ASTs. Then, we compute the tree edit distance between two trees using
the algorithm Treed~\cite{oopsla10}. Specifically, the tree edit
distance is calculated by number of operations ({\em add}, {\em
delete}, {\em replace}, and {\em move}) to make them identical.

We introduce a formula to normalize the edit distance so that it can
be used in our experiments. The normalized value is computed~as:
\[TREED = 1 -  \frac{TreeEditDistance\left(AST_R, AST_T\right)}{CountNodes \left(AST_R+AST_T\right)}\] 
  
where $TreeEditDistance\left(AST_R, AST_T\right)$ is the editing
distance between two trees $AST_R$ of reference code and $AST_T$ of
translated code; and the denominator is the total number of nodes in
both trees. The value of TREED is from 0 to 1.
%
For any two trees, there will always exist at least one editing (such
as the one that deletes all the nodes of the first tree and inserts all
the nodes of the second). Therefore, there will always exist at least
one TREED value and the higher value it is, the more similar those
trees are.

\begin{figure}[h]
	\caption{Tree Editing Example: In the label of each node, its type is in capital font and its val (if exists) is in normal font}
	\includegraphics[scale=0.3]{img/treed.png}
	\centering
	\label{fig:treed}
\end{figure}

In the example in Figure \ref{fig:treed}, an \textit{if} statement was
edited by modifying the \textit{if} branch and adding an \textit{else}
branch. The two ASTs represent the two versions of a method. An edit
consists of one \textit{Delete} (dotted line box), one \textit{Update}
(double-line box), and four \textit{Insert} operations (bold
boxes). Other nodes (single- line boxes) are either unchanged or
moved. Based on the formula of TREED, the result in this case is:
$TREED = 1 - \frac{1 + 1 + 4}{16}=0.625$.

\subsubsection{\textbf{Graph Vector Edit Distance (GVED)}}

Graph-based approaches in representing program semantics have become
popular. Among those approaches, PDGs are one of the most popular.  To
capture the graph structures in PDGs, we choose Exas~\cite{fase09}.
Exas is an efficient structural characteristic feature extraction
approach that approximates and captures the structure within the
fragments of artifacts~\cite{fase09}.  In our study, we use Exas as a
mean of computing the difference between two PDGs. Given a pair of
method in C\# which are need to be compared, their respective
(PDGs) are built.
% with some additional nodes from GROUM~\cite{fse09}.
Exas vectors will be computed on those graphs. In Exas, the
characteristic features are extracted from the patterns of elements of
the graphs. The code fragments are characterized by their counting
vectors of those features. The difference between two vectors reflects
the difference of two graphs.

%Therefore, distance of these counting vectors is considered the way to measure the sematic between code fragments.

Figure~\ref{fig:PDGs} shows the PDGs of the code fragments 1 and
2. These graphs are analysed by Exas, which focuses on two kinds of
patterns of structural information of the graph, called $\left(p,q\right)$-node
and $n$-path as can be seen in Table~\ref{tab:feature1} and
Table~\ref{tab:feature2}.

An efficient way to express the property ``having the same or similar
features'' is to use vectors. The characteristic vector of a fragment
is the occurrence-count vector of its features. That is, each position
in the vector is indexed for a feature and the value at that position
is the number of occurrences of that feature in the
fragment. Table~\ref{tab:featureIndex} shows the indexes of the
features, which are global across all vectors. Based on the occurrence
counts, the vectors for code fragment 1 and~2 are
$V_1$(1,1,1,1,1,0,1,0...) and $V_2$(1,1,0,1,1,1,1,1...),
respectively. Two fragments having the same feature sets and
occurrence counts will have the same vectors. The
vector similarity can be measured by a chosen vector distance such as
1-norm distance.

We introduce the formula for normalizing the result of vector edit
distance which is used in our experiments. The normalized
value is described as
\[GVED \left( V_1, V_2 \right) = 1 - \sum_{i=1}^{n} \frac{ \mid XV1_i - XV2_i \mid}{XV1_i + XV2_i}\]
where $n$ denotes the number of vector scalar, $V_1$ denotes the
counting vector of the first graph, $V_2$ denotes the counting vector
of the second graph; $XV1_i$ denotes the value of the ($i-th$) scalar
of $V_1$; and $XV2_i$ denotes the value of the ($i-th$) scalar of
$V_2$.

In this example in Figure~\ref{code1code2}, the value of GVED is
$GVED\left(V_1, V_2\right) = 1 - \frac{8 }{20} = 0.6 $.

\begin{figure}
\begin{lstlisting}[language=JAVA]
	Code 1:
	void foo(int i) {
		int j;
		if (i < 2) {
			j = 1;
		} else {
			j = 2;
		}
	}

	Code 2:
	void foo(int i) {
		int j;
		if (i < 2)
			j = i;	
		j = 2;
	}
\end{lstlisting}
\caption{Example of two code fragments}
\label{code1code2}
\end{figure}

\begin{figure}[t]
	\caption{An example: two PDGs represent code fragments 1 and 2}
	\includegraphics[scale=0.4]{img/Diagram_PDG.png}
	\centering
	\label{fig:PDGs}
\end{figure}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{Feature Table of Code Fragment 1 in Exas}
  \scalebox{0.65}{
    \begin{tabular}{|l|l|l|l|l|r|}
    \toprule
    \textbf{Pattern} & \multicolumn{5}{c|}{\textbf{Feature of Code1}} \\
    \midrule
    \textit{\textbf{1-path}} & inputInt & intSmall2 & intEqual1 & intEqual2 & \multicolumn{1}{l|}{declareInt} \\
    \midrule
    \textit{\textbf{2-path}} & \multicolumn{1}{p{6.415em}|}{inputInt-intSmall2} & \multicolumn{1}{p{5.915em}|}{intSmall2-intEqual1} & \multicolumn{1}{p{6em}|}{intSmall2-intEqual2} & \multicolumn{1}{p{5.75em}|}{declareInt-intEqual1} & \multicolumn{1}{p{5em}|}{declareInt-intEqual2} \\
    \midrule
    \textit{\textbf{3-path}} & \multicolumn{1}{p{6.415em}|}{intputInt-intSmall2-intEqual1} & \multicolumn{1}{p{5.915em}|}{intputInt-intSmall2-intEqual2} &       &       &  \\
    \midrule
    \textit{\textbf{(p,q)-node}} & inputInt-0-1 & intSmall2-1-2 & intEqual1-2-0 & intEqual2-1-2 &  \\
    \bottomrule
    \end{tabular}%
	}
  \label{tab:feature1}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
	\caption{Feature Table of Code Fragment 2 in Exas}
	\scalebox{0.65}{
	    \begin{tabular}{|l|l|l|l|l|r|}
    \toprule
    \textbf{Pattern} & \multicolumn{5}{c|}{\textbf{Feature of Code2}} \\
    \midrule
    \textit{\textbf{1-path}} & inputInt & intSmall2 & intEqualInt & intEqual2 & \multicolumn{1}{l|}{declareInt} \\
    \midrule
    \textit{\textbf{2-path}} & \multicolumn{1}{p{6.415em}|}{inputInt-intSmall2} & \multicolumn{1}{p{5.915em}|}{intSmall2-intEqualInt} & \multicolumn{1}{p{6em}|}{declareInt-intEqual1} & \multicolumn{1}{p{5.75em}|}{declareInt-intEqual2} &  \\
    \midrule
    \textit{\textbf{3-path}} & \multicolumn{1}{p{6.415em}|}{intputInt-intSmall2-intEqualInt} &       &       &       &  \\
    \midrule
    \textit{\textbf{(p,q)-node}} & inputInt-0-1 & intSmall2-1-1 & intEqualInt-2-0 & intEqual2-1-0 &  \\
    \bottomrule
    \end{tabular}%
	}
  \label{tab:feature2}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
	\centering
	\caption{Feature Indexing}
	\scalebox{0.75}{
	\begin{tabular}{|cccc|}
		\toprule
		\multicolumn{1}{|l|}{\textbf{Feature}} & \multicolumn{1}{l|}{\textbf{Index}} & \multicolumn{1}{l|}{\textbf{Counted in Code1}} & \multicolumn{1}{l|}{\textbf{Counted in Code2}} \\
		\midrule
		\multicolumn{1}{|l|}{inputInt} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{intSmall2} & \multicolumn{1}{r|}{2} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{intEqual1} & \multicolumn{1}{r|}{3} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{0} \\
		\midrule
		\multicolumn{1}{|l|}{intEqual2} & \multicolumn{1}{r|}{4} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{declareInt} & \multicolumn{1}{r|}{5} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{intEqualInt} & \multicolumn{1}{r|}{6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|p{5.75em}|}{inputInt-intSmall2} & \multicolumn{1}{r|}{7} & \multicolumn{1}{r|}{1} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{1}{|l|}{intEqual2-1-0} & \multicolumn{1}{r|}{8} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1} \\
		\midrule
		\multicolumn{4}{|c|}{To be continued} \\
		\bottomrule
	\end{tabular}%
	}
	\label{tab:featureIndex}%
\end{table}%





